TimbreTron: A WaveNet(CycleGAN(CQT(Audio))) Pipeline for Musical Timbre Transfer

In this work, we address the problem of musical timbre transfer, where the goal is to manipulate the timbre of a sound sample from one instrument to match another instrument while preserving other musical content, such as pitch, rhythm, and loudness. In principle, one could apply image-based style transfer techniques to a time-frequency representation of an audio signal, but this depends on having a representation that allows independent manipulation of timbre as well as high-quality waveform generation. We introduce TimbreTron, a method for musical timbre transfer which applies "image" domain style transfer to a time-frequency representation of the audio signal, and then produces a high-quality waveform using a conditional WaveNet synthesizer. We show that the Constant Q Transform (CQT) representation is particularly well-suited to convolutional architectures due to its approximate pitch equivariance. Based on human perceptual evaluations, we confirmed that TimbreTron recognizably transferred the timbre while otherwise preserving the musical content, for both monophonic and polyphonic samples.

==> macros.tex <==


% Evaluating ML estimators

% Notation
\newcommand{\prob}{\mathrm{Pr}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\variance}{\mathrm{Var}}
\newcommand{\dirichlet}{\mathrm{Dirichlet}}
\newcommand{\multinomial}{\mathrm{Multinomial}}
\newcommand{\normal}{{\cal N}}
\newcommand{\normalInfoForm}{{{\cal N}^{-1}}}
\newcommand{\inverseGamma}{{\mathrm{Gamma}^{-1}}}
\newcommand{\betaDist}{\mathrm{Beta}}
\newcommand{\bernoulli}{\mathrm{Bernoulli}}
\newcommand{\zeroVec}{\mathbf{0}}
\newcommand{\zeroMat}{\mathbf{0}}
\newcommand{\onesVec}{\mathbf{1}}
\newcommand{\ident}{\mathbf{I}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\entropy}{\mathcal{H}}
\newcommand{\kldiv}{{\mathrm{D}_{\rm KL}}}
\newcommand{\klBars}{{\,\|\,}}
\newcommand{\given}{{\hspace{.1em}|\hspace{.1em}}}
\DeclareMathOperator{\kvec}{vec}
\newcommand{\stackVec}[2]{{\left( \begin{array}{c} #1 \\ #2 \end{array} \right)}}
\newcommand{\stackMat}[4]{{\left( \begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array} \right)}}
\DeclareMathOperator{\tr}{tr}
\newcommand{\intD}{\textrm{d}}



% Dimensions
\newcommand{\ndata}{{N}}
\newcommand{\ntest}{{N_{test}}}
\newcommand{\nsamp}{{K}}
\newcommand{\ndist}{{T}}
\newcommand{\ncomp}{{K}}
\newcommand{\ndim}{{D}}


% Indices
\newcommand{\dataIdx}{{i}}
\newcommand{\somethingI}[2]{{#1_{#2}}}
\newcommand{\somethingJ}[2]{{#1_{#2}}}
\newcommand{\somethingIJ}[3]{{#1_{#2 #3}}}
\newcommand{\dimIdx}{{j}}
\newcommand{\latentIdx}{{k}}
\newcommand{\sampleIdx}{{k}}
\newcommand{\somethingS}[2]{{#1^{(#2)}}}
\newcommand{\somethingIS}[3]{{#1_{#2}^{(#3)}}}
\newcommand{\distIdx}{{t}}
\newcommand{\compIdx}{{k}}
\newcommand{\somethingK}[2]{{#1_{#2}}}
\newcommand{\somethingKJ}[3]{{#1_{#2 #3}}}
\newcommand{\nsStepIdx}{t}
\newcommand{\smallestSampleIdx}{\sampleIdx_\star}

% Distributions
\newcommand{\pmf}{{p}}
\newcommand{\pmfEstimate}{{\hat{p}}}
\newcommand{\pmfUnnorm}{{f}}
\newcommand{\pfn}{\mathcal{Z}}
\newcommand{\pmfProposal}{{q}}
\newcommand{\pmfProposalUnnorm}{{g}}
\newcommand{\distFamily}{\mathcal{P}}
\newcommand{\pfnTarget}{{\pfn_\pmf}}
\newcommand{\pfnTargetEstimate}{{\hat{\pfn}_\pmf}}
\newcommand{\pfnProposal}{{\pfn_\pmfProposal}}
\newcommand{\pmfAlternative}{{p^\prime}}
\newcommand{\pmfWI}{{\pmf_{wi}}}
\newcommand{\nsPrior}{\pi}
\newcommand{\nsConstrainedPrior}[1]{\breve{\nsPrior}_{#1}}
\newcommand{\nsLikelihood}{L}
\newcommand{\nsCutoff}{C}
\newcommand{\nsCutoffT}[1]{\nsCutoff_{#1}}
\newcommand{\nsVolume}{V}

% Generic state variables
\newcommand{\genState}{\mathbf{x}}
\newcommand{\genStateSpace}{\mathcal{X}}
\newcommand{\genStateS}[1]{{\somethingS{\genState}{#1}}}
\newcommand{\genStateUni}{{x}}
\newcommand{\rvGen}{\mathbf{x}}
\newcommand{\rvGenI}[1]{{\mathbf{x}^{(#1)}}}
\newcommand{\auxVarUni}{{u}}


% Observations
\newcommand{\obs}{\mathbf{y}}
\newcommand{\obsI}[1]{{\somethingI{\obs}{#1}}}
\newcommand{\obsIJ}[2]{{\somethingIJ{y}{#1}{#2}}}
\newcommand{\obsJ}[1]{{\somethingJ{\obs}{#1}}}
\newcommand{\obsMat}{\mathbf{Y}}
\newcommand{\obsMatIdx}[2]{{\obsMat_{#1,#2}}}
\newcommand{\obsMatSub}{{\tilde {\bf Y}}}
\newcommand{\latentObsMat}{\mathbf{X}}
\newcommand{\trainObsMat}{{\obsMat_{\rm obs}}}


% Parameters
\newcommand{\params}{{\boldsymbol \theta}}
\newcommand{\paramsSpace}{{\Theta}}
\newcommand{\paramsS}[1]{{\somethingS{\params}{#1}}}
\newcommand{\paramsI}[1]{{\params^{(#1)}}}
\newcommand{\paramsK}[1]{{\somethingK{\params}{#1}}}
\newcommand{\paramsMat}{{\boldsymbol \Theta}}


% Latent variables
\newcommand{\latent}{\mathbf{z}}
\newcommand{\latentI}[1]{{\somethingI{\latent}{#1}}}
\newcommand{\latentS}[1]{{\somethingS{\latent}{#1}}}
\newcommand{\latentIS}[2]{{\somethingIS{\latent}{#1}{#2}}}
\newcommand{\latentMat}{\mathbf{Z}}


% Generic model selection
\newcommand{\model}{\mathcal{M}}
\newcommand{\data}{\mathcal{D}}

% Generic estimators
\newcommand{\weightI}[1]{{w^{(#1)}}}
\newcommand{\weight}{{w}}
\newcommand{\weightS}[1]{{\somethingS{\weight}{#1}}}

% Generic matrix factorizations
\newcommand{\leftFactor}{\mathbf{U}}
\newcommand{\leftFactorRow}{\mathbf{u}}
\newcommand{\leftFactorRowI}[1]{{\mathbf{u}_{#1}}}
\newcommand{\leftFactorTrain}{{\leftFactor_{\rm obs}}}
\newcommand{\rightFactor}{\mathbf{V}}
\newcommand{\rightFactorColumnJ}[1]{{\mathbf{v}_{#1}}}
\newcommand{\noiseMat}{\mathbf{E}}
\newcommand{\noiseMatRow}{\mathbf{e}}
\newcommand{\noisePrec}{{\lambda}}
\newcommand{\noiseVar}{{\sigma^2_n}}
\newcommand{\leftFactorEntryIK}[2]{{u_{#1 #2}}}
\newcommand{\RightFactorEntryKJ}[2]{{v_{#1 #2}}}




% Matrix decomposition expressions
\newcommand{\gComp}{\mathsf{G}}
\newcommand{\mComp}{\mathsf{M}}
\newcommand{\bComp}{\mathsf{B}}
\newcommand{\cComp}{\mathsf{C}}

\newcommand{\threshold}{\mathrm{T}}


\newcommand{\pmfPredictive}{{\pmf_{\rm pred}}}
\newcommand{\pmfPredictiveApprox}{{\tilde{p}_{\rm pred}}}







% general partition function estimation


\newcommand{\pfnEstimate}{{\hat \pfn}}
\newcommand{\pfnEstimateSIS}{{\pfn_{SIS}}}

% importance sampling


% AIS
\newcommand{\pmfProposalForward}{{\pmfProposal_{for}}}
\newcommand{\pmfProposalBackward}{{\pmfProposal_{back}}}
\newcommand{\invTemp}{{\beta}}
\newcommand{\trans}{\mathcal{T}}
\newcommand{\transReverse}{\tilde{\mathcal{T}}}
\newcommand{\succState}{{\genState^\prime}}

% SMC
\newcommand{\sumOfWeights}{{S}}

% Chib's method
\newcommand{\latentPointEstimate}{{\latent^\star}}
\newcommand{\paramsPointEstimate}{{\params^\star}}
\newcommand{\leftFactorPointEstimate}{{\leftFactor^\star}}
\newcommand{\rightFactorPointEstimate}{{\rightFactor^\star}}

% variational
\newcommand{\pmfVariational}{{q}}
\newcommand{\variationalFunc}{\mathcal{F}}

% relationship with inference
\newcommand{\auxiliary}{\mathbf{v}}

% clustering
\newcommand{\mixtureProb}{{\boldsymbol \pi}}
\newcommand{\mixtureProbK}[1]{{\somethingK{\pi}{#1}}}
\newcommand{\dirichletParam}{{\alpha}}
\newcommand{\mixtureMeanK}[1]{\somethingK{{\boldsymbol \mu}}{#1}}
\newcommand{\mixtureMeanKJ}[2]{\somethingKJ{\mu}{#1}{#2}}
\newcommand{\mixtureParamsMean}{{\boldsymbol \mu}}
\newcommand{\mixtureMuVar}{{\sigma^2_\mixtureParamsMean}}
\newcommand{\mixtureBetweenVar}{{s^2}}
\newcommand{\mixtureBetweenVarInv}{{s^{-2}}}
\newcommand{\mixtureVarKJ}[2]{{\sigma^2_{#1 #2}}}
\newcommand{\mixtureVarKJInv}[2]{{\sigma^{-2}_{#1 #2}}}
\newcommand{\mixtureParams}{{\params}}
\newcommand{\mixtureParamsK}[1]{{\params_{#1}}}
\newcommand{\assignmentI}[1]{\somethingI{z}{#1}}


% factor analysis
\newcommand{\faCompVar}{{{\boldsymbol \sigma}^2_f}}
\newcommand{\faCompVarK}[1]{{\sigma^2_{f #1}}}
\newcommand{\faObsVar}{{{\boldsymbol \sigma}^2_n}}
\newcommand{\faObsVarJ}[1]{{\sigma^2_{n #1}}}
\newcommand{\faFactors}{{\boldsymbol \Theta}}
\newcommand{\faFactorsK}[1]{{{\boldsymbol \theta}_{#1}}}
\newcommand{\gammaParamOne}{{a}}
\newcommand{\gammaParamTwo}{{b}}
\newcommand{\faMean}{{\boldsymbol \mu}}
\newcommand{\faMeanVar}{{\sigma^2_\faMean}}


% Probabilistic matrix factorization
\newcommand{\pmfInput}{\mathbf{X}}
\newcommand{\pmfInputEntry}{{x}}
\newcommand{\pmfFacOne}{\mathbf{U}}
\newcommand{\pmfFacOneEntry}{{u}}
\newcommand{\pmfFacTwo}{\mathbf{V}}
\newcommand{\pmfFacTwoEntry}{{v}}
\newcommand{\pmfFeaturePrec}{{\boldsymbol \eta}}
\newcommand{\pmfFeaturePrecEntry}{{\eta}}
\newcommand{\pmfNoisePrec}{{\lambda}}
\newcommand{\pmfFeatureA}{{a}}
\newcommand{\pmfFeatureB}{{b}}
\newcommand{\pmfNoiseA}{{a^\prime}}
\newcommand{\pmfNoiseB}{{b^\prime}}

% binary latent features
\newcommand{\binProb}{{\boldsymbol \pi}}
\newcommand{\binProbK}[1]{{\pi_{#1}}}
\newcommand{\binAttrMat}{\mathbf{Z}}
\newcommand{\binAttrMatIdx}[2]{{\binAttrMat_{#1,#2}}}
\newcommand{\binAttrMatIdxTransp}[2]{{\binAttrMat_{#1,#2}^T}}
\newcommand{\binAttrI}[1]{{\mathbf{z}_{#1}}}
\newcommand{\binAttrIK}[2]{{z_{#1 #2}}}
\newcommand{\binBias}{\mathbf{b}}
\newcommand{\binFeaturesMat}{\mathbf{A}}
\newcommand{\binFeaturesK}[1]{{{\bf a}_{#1}}}
\newcommand{\binFeaturesJ}[1]{{{\bf a}_{#1}}}
\newcommand{\binFeatureVar}{{\sigma^2_f}}
\newcommand{\binFeatureVarInv}{{\sigma^{-2}_f}}
\newcommand{\binObsVar}{{\sigma^2_n}}
\newcommand{\binObsVarInv}{{\sigma^{-2}_n}}
\newcommand{\binBiasVar}{{\sigma^2_b}}
\newcommand{\betaParamOne}{{a}}
\newcommand{\betaParamTwo}{{b}}
\newcommand{\binMean}{{\boldsymbol \mu}}
\newcommand{\binMeanVar}{{\sigma^2_\faMean}}

\newcommand{\TODO}[1]{{\color{red} [[TODO: #1]]}}


% Gaussian distribution
\newcommand{\gaussMean}{{\boldsymbol \mu}}
\newcommand{\gaussMeanK}[1]{{\somethingK{\gaussMean}{#1}}}
\newcommand{\gaussCov}{{\boldsymbol \Sigma}}
\newcommand{\gaussCovK}[1]{{\somethingK{\gaussCov}{#1}}}




\newcommand{\mhRatio}{{r}}


% Compositional importance sampling




\newcommand{\statGen}{{h}}
\newcommand{\aisWeight}{{w}}


\DeclareMathOperator{\chol}{chol}

\DeclareMathOperator*{\var}{var}
\DeclareMathOperator*{\cov}{cov}

% Moment averaging
\newcommand{\pmfOne}{{\pmf_a}}
\newcommand{\pmfTwo}{{\pmf_b}}
\newcommand{\pmfUnnormOne}{{\pmfUnnorm_a}}
\newcommand{\pmfUnnormTwo}{{\pmfUnnorm_b}}
\newcommand{\pfnOne}{{\pfn_a}}
\newcommand{\pfnTwo}{{\pfn_b}}
\newcommand{\pfnTwoEstimate}{{\hat{\pfn}_b}}

\newcommand{\dParams}{{\dot \params}}
\newcommand{\pathParam}{{\beta}}
\newcommand{\fisher}{{\bf G}}
\newcommand{\costFunc}{{\cal F}}
\newcommand{\distPath}{{\gamma}}
\newcommand{\natParams}{{\boldsymbol \eta}}
\newcommand{\expSuff}{{\bf s}}
\newcommand{\geomPath}{{\distPath_{GA}}}
\newcommand{\momentsPath}{{\distPath_{MA}}}
\newcommand{\momentsSplinePath}{{\distPath_{MAS}}}
\newcommand{\dNatParams}{{\dot \natParams}}
\newcommand{\dExpSuff}{{\dot \expSuff}}
\newcommand{\knotIdx}{{j}}
\newcommand{\nknots}{{R}}
\newcommand{\pathParamTwo}{{t}}
\newcommand{\distPathOpt}{{\distPath^*}}
\newcommand{\pathLength}{{\ell}}
\newcommand{\alloc}{{\ndist}}
\newcommand{\distPathTemp}{{\distPath^\prime}}
\newcommand{\bias}{{\delta}}

\newcommand{\varDist}{{q}}

\newcommand{\rbad}{{CD1(500) }}
\newcommand{\cnet}{{PCD(500) }}
\newcommand{\rgood}{{CD25(500) }}
\newcommand{\rsmall}{{CD1(20) }}
\newcommand{\csmall}{{PCD(20) }}

\newcommand{\partition}{{\stateSpace}}
\newcommand{\npartitions}{{N}}
\newcommand{\partitionIdx}{{j}}


\newcommand{\efNormState}{{h}}
\newcommand{\suff}{\mathbf{g}}
\newcommand{\mgMean}{{\boldsymbol \mu}}
\newcommand{\mgCov}{{\boldsymbol \Sigma}}
\newcommand{\mgPrec}{{\boldsymbol \Lambda}}
\newcommand{\mgPot}{\mathbf{h}}

\newcommand{\visUnits}{\mathbf{v}}
\newcommand{\hidUnits}{\mathbf{h}}
\newcommand{\visBiases}{\mathbf{a}}
\newcommand{\hidBiases}{\mathbf{b}}
\newcommand{\rbmWeights}{\mathbf{W}}

\newcommand{\gMeanOne}{{\mu_a}}
\newcommand{\gMeanTwo}{{\mu_b}}
\newcommand{\gStd}{{\sigma}}
\newcommand{\gaussDistance}{{d}}


% Moment averaging appendix
\newcommand{\step}{{h}}
\newcommand{\tempFn}{{H}}
\newcommand{\lagrangian}{\mathcal{L}}
\newcommand{\lmult}{{\lambda}}
\newcommand{\natParamsI}{{\eta}}
\newcommand{\suffI}{{g}}

\newcommand{\mean}{{\mu}}
\newcommand{\dMean}{{\dot \mu}}
\newcommand{\std}{{\sigma}}
\newcommand{\dStd}{{\dot \std}}
\newcommand{\precision}{{\lambda}}
\newcommand{\dPrecision}{{\dot \lambda}}
\newcommand{\potUni}{{\bf h}}
\newcommand{\dPotUni}{{\dot h}}
\newcommand{\secMt}{{s}}
\newcommand{\dSecMt}{{\dot s}}
\newcommand{\uniState}{{x}}

\newtheorem{theorem}{Theorem}


% Toy problem in introduction
\newcommand{\toySequence}{\mathcal{S}}
\newcommand{\toyExpression}{\mathcal{E}}
\newcommand{\toyRandom}{\mathsf{R}}
\newcommand{\toyCumsum}{\mathtt{cumsum}}
\newcommand{\toySquare}{\mathtt{square}}
\newcommand{\toyNthprime}{\mathtt{nthprime}}


% CIS derivations
\newcommand{\uParams}{{\boldsymbol \theta}}
\newcommand{\vParams}{{\boldsymbol \eta}}
\newcommand{\priorCovU}{{{\boldsymbol \Sigma}_\leftFactor}}
\newcommand{\priorCovV}{{{\boldsymbol \Sigma}_\rightFactor}}
\newcommand{\rightFactorCenters}{{\boldsymbol \Xi}}
\newcommand{\rightFactorAssignments}{{\bf Z}}
\newcommand{\rightFactorNoise}{{\bf E}}
\newcommand{\rightFactorCenterVar}{{\xi}}
\newcommand{\pmfLin}{{\pmf_{\rm lin}}}
\newcommand{\pmfProposalLin}{{\pmfProposal_{\rm lin}}}
\newcommand{\pmfProposalSecondOrder}{\pmfProposal_{\rm so}}
\newcommand{\pmfSecondOrder}{\pmf_{\rm so}}
\newcommand{\constraint}{{\phi}}
\newcommand{\pmfTarget}{\pmf}
\newcommand{\pmfPost}{{\pmf_{\rm post}}}
\newcommand{\pmfProposalPost}{{\pmfProposal_{\rm post}}}
\newcommand{\termOne}{{\mathcal{T}_1}}
\newcommand{\termTwo}{{\mathcal{T}_2}}
\newcommand{\termThree}{{\mathcal{T}_3}}
\newcommand{\flipMat}{{\bf F}}
\newcommand{\residMat}{{\bf R}}
\newcommand{\residMatPerp}{\residMat_{\perp}}


\newcommand{\uVar}{{\bf u}}
\newcommand{\vVar}{{\bf v}}
\newcommand{\pot}{{\bf h}}
\newcommand{\potU}{{\pot_\uVar}}
\newcommand{\potV}{\pot_\vVar}
\newcommand{\precUU}{{\bf A}}
\newcommand{\precUUInv}{{{\bf A}^{-1}}}
\newcommand{\precUV}{{\bf B}}
\newcommand{\precVU}{{{\bf B}^T}}
\newcommand{\precVVProposal}{{{\bf C}_\pmfProposal}}
\newcommand{\precVVProposalInv}{{{\bf C}_\pmfProposal^{-1}}}
\newcommand{\precVVTarget}{{{\bf C}_\pmfTarget}}
\newcommand{\precVVTargetInv}{{{\bf C}_\pmfTarget^{-1}}}
\newcommand{\vMeanProposal}{{{\boldsymbol \mu}_\pmfProposal}}
\newcommand{\vMeanProposalTransp}{{{\boldsymbol \mu}_\pmfProposal^T}}
\newcommand{\vMeanTarget}{{{\boldsymbol \mu}_\pmfTarget}}
\newcommand{\vMeanTargetTransp}{{{\boldsymbol \mu}_\pmfTarget^T}}
\newcommand{\expectProposal}{{\expect_\pmfProposalPost}}
\newcommand{\expectTarget}{{\expect_\pmfPost}}
\newcommand{\covU}{{{\boldsymbol \Sigma}_\uVar}}
\newcommand{\covV}{{{\boldsymbol \Sigma}_\vVar}}
\newcommand{\meanDiff}{{{\boldsymbol \Delta}_{\boldsymbol \mu}}}
\newcommand{\meanDiffTransp}{{{\boldsymbol \Delta}_{\boldsymbol \mu}^T}}
\newcommand{\redGreenMat}{{\bf Z}}


\newcommand{\leftFactorInit}{{{\bf U}_{\! 0}}}
\newcommand{\rightFactorInit}{{{\bf V}_{\! 0}}}
\newcommand{\leftFactorInitTransp}{{{\bf U}_{\! 0}^T}}
\newcommand{\rightFactorInitTransp}{{{\bf V}_{\! 0}^T}}
\newcommand{\constraintWeight}{{\nu}}
\newcommand{\innerStructurePrecMax}{{\gamma}}
\newcommand{\priorPrecU}{{\boldsymbol \Lambda}_{\leftFactor}}
\newcommand{\priorPrecUInv}{{\boldsymbol \Lambda}_{\leftFactor}^{-1}}
\newcommand{\priorPrecV}{{\boldsymbol \Lambda}_{\rightFactor}}
\newcommand{\priorPrecVInv}{{\boldsymbol \Lambda}_{\rightFactor}^{-1}}
\newcommand{\priorPrecVEmpirical}{\hat{\boldsymbol \Lambda}_\rightFactor}
\newcommand{\innerStructure}{{\boldsymbol S}}
\newcommand{\innerStructurePerp}{\innerStructure_{\! \perp}}
\newcommand{\leftProjMat}{{{\bf P}_\leftFactor}}
\newcommand{\leftProjMatReg}{{{\bf \tilde{P}}_\leftFactor}}
\newcommand{\leftPseudo}{{\tilde {\bf U}}}
\newcommand{\leftPseudoTransp}{{\tilde {\bf U}^T}}
\newcommand{\leftBasis}{\TODO[left basis]}
\newcommand{\leftBasisPerp}{\TODO[left basis]}
\newcommand{\rightBasis}{{\bf Q}}
\newcommand{\rightBasisPerp}{{\bf \bar{R}}}
\newcommand{\rightBasisKron}{{{\bf R}_{\otimes}}}
\newcommand{\rightBasisKronTransp}{{{\bf R}_{\otimes}^T}}
\newcommand{\leftVarK}[1]{{\sigma^2_{#1}}}
\newcommand{\leftVarKInv}[1]{{\sigma^{-2}_{#1}}}

\newcommand{\precVVProposalRar}{{{\bf \tilde{C}}_q}}
\newcommand{\precVVProposalRarInv}{{{\bf \tilde{C}}_q^{-1}}}
\newcommand{\precVVTargetRar}{{{\bf \tilde{C}}_p}}
\newcommand{\precVVTargetRarInv}{{{\bf \tilde{C}}_p^{-1}}}
\newcommand{\innerStructureRar}{{\bf \tilde{S}}}
\newcommand{\innerStructureRarCC}{{{\bf \tilde{S}}_{CC}}}
\newcommand{\innerStructureRarCCInv}{{{\bf \tilde{S}}_{CC}^{-1}}}
\newcommand{\innerStructureRarCN}{{{\bf \tilde{S}}_{CN}}}
\newcommand{\innerStructureRarNC}{{{\bf \tilde{S}}_{NC}}}
\newcommand{\innerStructureRarNN}{{{\bf \tilde{S}}_{NN}}}
\newcommand{\innerStructureRarNNInv}{{{\bf \tilde{S}}_{NN}^{-1}}}
\newcommand{\rarCC}{{\bf D}}
\newcommand{\rarCN}{{{\bf F}^T}}
\newcommand{\rarNC}{{\bf F}}
\newcommand{\rarNN}{{\bf E}}
\newcommand{\tempRarMat}{{\bf G}}
\newcommand{\subCC}{{CC}}
\newcommand{\jMat}{{\bf J}}
\newcommand{\kMat}{{\bf K}}
\newcommand{\lMat}{{\bf L}}
\newcommand{\mMat}{{\bf M}}

\newcommand{\transMat}{{\bf T}}
\newcommand{\transMatDelta}{{{\Delta}_\transMat}}
\newcommand{\rotMat}{{\bf Q}}
\newcommand{\transMatOne}{\transMat_1}
\newcommand{\transMatTwo}{\transMat_2}
\newcommand{\constraintViolation}{{\bf D}}
\newcommand{\leftFactorTransformed}{{\leftFactor^{(\transMat)}}}
\newcommand{\rightFactorTransformed}{{\rightFactor^{(\transMat)}}}
\newcommand{\priorPrecUTransformed}{{{\boldsymbol \Lambda}_{\leftFactor}^{(\transMat)}}}
\newcommand{\priorPrecVTransformed}{{{\boldsymbol \Lambda}_{\rightFactor}^{(\transMat)}}}

\newcommand{\rightFactorRowSpace}{\rightFactor_{\rm row}}
\newcommand{\rightFactorPerp}{\rightFactor_{\! \perp}}
\newcommand{\rightFactorProjPerp}{\tilde{\rightFactor}_{\! \perp}}

\newcommand{\priorPrecVTrans}{{{\bf \tilde{\Lambda}}_\rightFactor}}

\newcommand{\potVMessage}{{\bf h}_{\uVar \rightarrow \vVar}}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

